Understanding the Effectiveness of Ultrasonic Microphone Jammer

Recent works have explained the principle of using ultrasonic transmissions to jam nearby microphones. These signals are inaudible to nearby users, but leverage "hardware nonlinearity" to induce a jamming signal inside microphones that disrupts voice recordings. This has great implications on audio privacy protection. In this work, we gain a deeper understanding on the effectiveness of ultrasonic jammer under practical scenarios, with the goal of disabling both visible and hidden microphones in the surrounding area. We first experiment with existing jammer designs (both commercial products and that proposed by recent papers), and find that they all offer limited angular coverage, and can only target microphones in a particular direction. We overcome this limitation by building a circular transducer array as a wearable bracelet. It emits ultrasonic signals simultaneously from many directions, targeting surrounding microphones without needing to point at any. More importantly, as the bracelet moves with the wearer, its motion increases jamming coverage and diminishes blind spots (the fundamental problem facing any transducer array). We evaluate the jammer bracelet under practical scenarios, confirming that it can effectively disrupt visible and hidden microphones in the surrounding areas, preventing recognition of recorded speech. We also identify limitations and areas for improvement.

==> Makefile <==

LATEX=latex #--synctex=1

BIBTEX=bibtex
BIBFILE=ultra.bib
PAPER=ultra

PDFLATEXFLAGS = #--synctex=1

TEXFILES = ultra.tex \
	1.intro.tex \
	2.related.tex \
	3.jamming-eval2.tex\
	4.wearable.tex \
	5.prototype.tex \
	6.eval2.tex \
	7.discussion.tex \
	8.conclusion.tex 

EPSFIGS = $(wildcard plots/*.eps) \
          $(wildcard plots/*/*.eps) \
          $(wildcard figs/*/*.eps) \
          $(wildcard figs/*.eps) \
          $(wildcard figs_wn/*.eps) \
          $(wildcard figs_wn/*/*.eps) \
          $(wildcard figs_new/*.eps) \
          $(wildcard figs_new/*/*.eps) \
          $(wildcard figs_new/*/*/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) $(PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

# $(PAPER).pdf: $(PAPER).dvi
# 	dvipdf $(PAPER).dvi

# %.pdf:  %.tex   acmart.cls ACM-Reference-Format.bst
# 	pdflatex $(PDFLATEXFLAGS) $<
# 	- bibtex $*
# 	pdflatex $(PDFLATEXFLAGS) $<
# 	pdflatex $(PDFLATEXFLAGS) $<
# 	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
# 	do pdflatex $(PDFLATEXFLAGS) $<; done

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.pdf *.out *.synctex.gz figs/*.pdf plots/*.pdf

